FedCAR: Cross-client Adaptive Re-weighting for Generative Models in Federated Learning

Generative models trained on multi-institutional datasets can provide an enriched understanding through diverse data distributions. However, training the models on medical images is often challenging due to hospitals' reluctance to share data for privacy reasons. Federated learning(FL) has emerged as a privacy-preserving solution for training distributed datasets across data centers by aggregating model weights from multiple clients instead of sharing raw data. Previous research has explored the adaptation of FL to generative models, yet effective aggregation algorithms specifically tailored for generative models remain unexplored. We hereby propose a novel algorithm aimed at improving the performance of generative models within FL. Our approach adaptively re-weights the contribution of each client, resulting in well-trained shared parameters. In each round, the server side measures the distribution distance between fake images generated by clients instead of directly comparing the Fr\'echet Inception Distance per client, thereby enhancing efficiency of the learning. Experimental results on three public chest X-ray datasets show superior performance in medical image generation, outperforming both centralized learning and conventional FL algorithms. Our code is available at https://github.com/danny0628/FedCAR.

==> sections/introduction.tex <==
\section{Introduction}
%\subsection{Federated learning with generative model}

% by jh
%Federated learning (FL) is one of the machine learning approaches that is designed to train a model across multiple clients without migration of data to the central server. As the training data remains on the local clients, FL is particularly valuable in contexts where data security is crucial, such as in healthcare institutions. 
% 생성 모델
%Oneof the famous generative architectures is Generative Adversarial Network (GAN)  which was introduced by Ian Goodfellow in 1994. Since its invention it has achieved tremendous improvement in computer vision especially in image-translation and image-generation. Despite the remarkable performance, GAN has a specific limitation when it deals with a smaller dataset. It is well known that GAN with training abundant data can generate high-quality outcomes while inadequate data shows significant degradation in the quality of generated results. 



% by mj
% FL과 PS에 대한 기본 설명
Federated Learning (FL) is a machine learning framework designed to train models directly on clients' devices without data migration or centralization. Within FL, the central server iteratively aggregates weights from local clients into a single weight and redistributes it to local clients where the training data remains securely.
% FL의 decentralized nature는 의료분야에 많이 쓰임 + GAN-FL이 주목받음
The decentralized nature of FL offers a significant advantage in contexts where data security is crucial, such as in healthcare institutions, leading to its widespread use in medical image analysis \cite{Wicaksana2022FedMixMS, Wu2022FedRareFL, MRImageRecon, SplitAVG, Jiang2021HarmoFLHL}. Recently, generative adversarial network (GAN)\cite{Goodfellow2014GenerativeAN} within FL has drawn attentions for their remarkable versatility across various applications such as data anonymization\cite{Piacentino2024GeneratingF}, cross-domain adaptations \cite{Peng2020Federated} and other unsupervised learning tasks\cite{Das2022FGANFG, Ke2021StyleN}, all while preserving privacy.
% 하지만 메디컬 데이터셋은 작고, non-iid에서는 안되는 경향이 있음
However, adaptation of GAN within FL systems face two significant challenges. Initially, medical imaging datasets often suffer from limitations in size and data availability. It is well known that GAN with training abundant data can generate high-quality outcomes while inadequate data shows significant degradation in the quality of generated results. Furthermore, FL generally does not guarantee its performance in the circumstance of non-independent and identically distributed data(non-iid) \cite{Zhao2018FederatedLN, Li2022FederatedLG, math11194123, Zeng2022AdaptiveFLN}. In practical scenarios, medical datasets from various sites often exhibit considerable discrepancy in data distributions. %, referred to as data heterogeneity.

% 문제 해결을 위해 새로운 aggregation algorithm을 제안
To overcome these challenges, we propose a novel algorithm solely designed for generative models within FL frameworks. Our method includes adaptive re-weighting the contributions of client models based on quantitative evaluation of distribution discrepancies across clients. Our strategy maximizes learning efficiency by reassigning weights to clients that learned representations well at each round. We conducted experiments to show this approach can significantly improve performance of generative model. In addition, while conventional aggregation algorithms like FedAvg may tend to excessively overlook clients with smaller datasets, our approach avoids such issues by solely relying on clients' generative capabilities.

% privacy 얘기 쓰기 

% Parameter server 설명
%The central server, or parameter server (PS), originally introduced for large-scale distributed training \cite{Dean2012LargeSD} and privacy-preserving training \cite{Shokri2015PrivacypreservingDL}, plays a pivotal role in FL.


==> sections/relatedworks.tex <==
% \subsection{Related works}


% FL-GAN (augmentation ....)
%There are several studies explored potential benefits of federated learning in GAN and proved that it can converge even with non-i.i.d. situations. However, to our knowledge, none of them released the source code. The idea of federated GAN is similar to normal federated learning except they share two kinds of weights: discriminator and generator. 
The concept of federated learning adapted to GAN has been already explored on distributed data settings, both in iid \cite{Hardy2018MDGANMG} and non-iid settings \cite{Yonetani2019DecentralizedLO}. Recently, FedGAN\cite{Rasouli2020FedGANFG} was introduced by training local generators and discriminators synchronously through a parameter server, as studied also in \cite{10.1007/978-3-030-60636-7_1}.
% FL aggregation algorithms
FedAvg\cite{McMahan2016CommunicationEfficientLO} is a widely used FL aggregation method known for its simplicity and effectiveness. This approach is also applied in FedGAN \cite{Rasouli2020FedGANFG} by averaging client updates on a parameter server. FedOpt\cite{reddi2021adaptive} enhances FedAvg by incorporating adaptive optimization techniques, such as ADAGRAD, ADAM, or YOGI. In \cite{Han2023FedMLSecurityAB}, FedOpt was implemented as the aggregation algorithm for training GAN within FL systems for better handling of non-IID datasets. Building upon this foundation, our method further extends the capabilities of FedGAN by dynamically reweighting contributions of clients during aggregation.



==> tables/table.tex <==
% \begin{table}[ht]
% \caption{Performance comparison result within the i.i.d. scenario that randomly selected data from NIH, Stanford and VIN datasets are equally distributed to three clients.}
% \centering
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{4}{c}{i.i.d} \\
% \cmidrule(r){2-5}
% Method & client1 & client2 & client3 & Avg. \\
% \midrule
% Centralized & - & - & - & 8.58 \\ 
% Individual & 35 & 29.45 & & \\
% FedAvg \cite{McMahan2016CommunicationEfficientLO} & 12.47 & 13.12 & 11.85 &   \\
% FedAdam \cite{reddi2021adaptive} & 23.22 & 24.96 & 21.92 &   \\
% \textbf{FedCAR(Ours)} & 63.00 & 68.94 & 60.75 & \\
% \bottomrule
% \end{tabular}
% \label{tab:my_label}
% \end{table}

% \begin{table}
% \caption{Performance comparison result within the i.i.d. scenario that randomly selected data from NIH, Stanford and VIN datasets are equally distributed to three clients.}
% \end{table}


% \begin{table}
% \caption{Performance comparison result within the mild non-i.i.d. scenario that each client possesses an identical quantity of data yet characterized by distinct attributes.}
% \begin{center}
% \setlength{\tabcolsep}{12pt}
% \renewcommand{\arraystretch}{1.35}
% \begin{NiceTabular}{wc{2cm}wc{1cm}*{5}{c}}
% \toprule
% \Block{2-2}{Method} & & \Block{1-4}{Dataset} \\
% \cmidrule{3-7}  
% &  & NIH & Stanford & VIN & Average & \\

% \midrule
% conv30000 & &  &  &  & 8.58                   \\
% conv10000 & & 11.87 & 12.76 & 5.49 & 10.04                   \\
% FedAvg & & 7.59 & 10.59 & 6.23 & 8.13                   \\
% FedAdam & & 8.13 & 10.54 & 6.18 & 8.28           \\
% FedYogi & & 36.90 & 50.27 & 23.89 & xx                   \\
% \hline
% \textbf{FedCAR(Ours)} & & 6.62 & 9.8 & 4.94 & 7.12                  \\
% \bottomrule
% \end{NiceTabular}
% \end{center}
% \end{table}
